Streaming and Query Once Space Complexity of Longest Increasing Subsequence

Longest Increasing Subsequence (LIS) is a fundamental problem in combinatorics and computer science. Previously, there have been numerous works on both upper bounds and lower bounds of the time complexity of computing and approximating LIS, yet only a few on the equally important space complexity. In this paper, we further study the space complexity of computing and approximating LIS in various models. Specifically, we prove non-trivial space lower bounds in the following two models: (1) the adaptive query-once model or read-once branching programs, and (2) the streaming model where the order of streaming is different from the natural order. As far as we know, there are no previous works on the space complexity of LIS in these models. Besides the bounds, our work also leaves many intriguing open problems.

==> references_copy.tex <==
@string{stoc05="Proceedings of the 37th Annual ACM Symposium on Theory of Computing"}

@IEEEtranBSTCTL{IEEEexample:BSTcontrol,
CTLdash_repeated_names= "no",
}

@inproceedings{Li:CCC:2011, 
  author    = {Li, Xin},
  title     = {A New Approach to Affine Extractors and Dispersers},
  booktitle = {Proceedings of the 26th Annual {IEEE} Conference on Computational
               Complexity, {CCC}},
  year      = {2011}
}

@inproceedings{ChattopadhyayL:stoc:2017,
  author    = {Eshan Chattopadhyay and
               Xin Li},
  editor    = {Hamed Hatami and
               Pierre McKenzie and
               Valerie King},
  title     = {Non-malleable codes and extractors for small-depth circuits, and affine
               functions},
  booktitle = {Proceedings of the 49th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2017, Montreal, QC, Canada, June 19-23, 2017},
  pages     = {1171--1184},
  publisher = {{ACM}},
  year      = {2017},
  url       = {https://doi.org/10.1145/3055399.3055483},
  doi       = {10.1145/3055399.3055483},
  timestamp = {Sun, 02 Jun 2019 21:10:31 +0200},
  biburl    = {https://dblp.org/rec/conf/stoc/Chattopadhyay017.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Li:focs:2012,  
    author      = {Li, Xin},  
    booktitle   = {2012 IEEE 53rd Annual Symposium on Foundations of Computer Science},   
    title       = {Non-malleable Extractors, Two-Source Extractors and Privacy Amplification}, 
    year        = {2012}
}

@inproceedings{Zuckerman:toc:2007,
    author      = {Zuckerman, David},
    title       = {Linear Degree Extractors and the Inapproximability of Max Clique and Chromatic Number},
    booktitle    = {Theory of Computing},
    year        = {2007}
}

@inproceedings{Zuc:random:1997,
    author      = {Zuckerman, David},
    title       = {Randomness-Optimal Oblivious Sampling},
    booktitle   = {Random Struct. Algorithms},
    year        = {1997}
}

@inproceedings{BarakKSSW05,
    Author = {Boaz Barak and Guy Kindler and Ronen Shaltiel and Benny Sudakov         and Avi Wigderson},
    Booktitle = stoc05,
    Pages = {1--10},
    Title = {Simulating Independence:  New Constructions of         Condensers, {R}amsey Graphs, Dispersers, and Extractors},
    Year = {2005}}

@inproceedings{Raz05,
    Author = {Ran Raz},
    Booktitle = stoc05,
    Pages = {11--20},
    Title = {Extractors with Weak Random Seeds},
    Year = {2005}}

@inproceedings{BhattacharyyaKSSZ10,
  author    = {Arnab Bhattacharyya and
               Swastik Kopparty and
               Grant Schoenebeck and
               Madhu Sudan and
               David Zuckerman},
  title     = {Optimal Testing of Reed-Muller Codes},
  booktitle = {51th Annual {IEEE} Symposium on Foundations of Computer Science, {FOCS}
               2010, October 23-26, 2010, Las Vegas, Nevada, {USA}},
  pages     = {488--497},
  publisher = {{IEEE} Computer Society},
  year      = {2010},
  url       = {https://doi.org/10.1109/FOCS.2010.54},
  doi       = {10.1109/FOCS.2010.54},
  timestamp = {Tue, 14 Jun 2022 13:12:40 +0200},
  biburl    = {https://dblp.org/rec/conf/focs/BhattacharyyaKSSZ10.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{v004a007,
 author = {Viola, Emanuele and Wigderson, Avi},
 title = {Norms, XOR Lemmas, and Lower Bounds for Polynomials and Protocols},
 year = {2008},
 pages = {137--168},
 doi = {10.4086/toc.2008.v004a007},
 publisher = {Theory of Computing},
 journal = {Theory of Computing},
 volume = {4},
 number = {7},
 URL = {https://theoryofcomputing.org/articles/v004a007},
}

@MISC{BISW04,
  author = {Boaz Barak and  Russel Impagliazzo and Amir Shpilka and Avi Wigderson},
  title = {Definition and existence of dimension expanders},
  year = {2004},
  howpublished={Discussion (no written record)}
}


@article{Bourgain09,
	Author = {Jean Bourgain},
	Journal = {Comptes Rendus Mathematique},
	Number = {7},
	Pages = {357-362},
	Title = {Expanders and dimensional expansion},
	Volume = {347},
	Year = {2009}}

@article{BourgainY13,
	Author = {Bourgain, Jean and Yehudayoff, Amir},
	Journal = {Geometric and Functional Analysis},
	Number = {1},
	Pages = {1--41},
	Title = {Expansion in {$SL_2(\mathbb{R})$} and monotone expanders},
	Volume = {23},
	Year = {2013}}

@inproceedings{cheng2018randomness,
  title={Randomness Extraction in AC0 and with Small Locality},
  author={Cheng, Kuan and Li, Xin},
  booktitle={Approximation, Randomization, and Combinatorial Optimization. Algorithms and Techniques (APPROX/RANDOM 2018)},
  year={2018},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@article{papakonstantinou2016true,
  title={True Randomness from Big Data},
  author={Papakonstantinou, Periklis A and Woodruff, David P and Yang, Guang},
  journal={Scientific reports},
  volume={6},
  pages = {33740},
  year={2016},
  publisher={Nature Publishing Group}
}


@article{DvirS11,
	Author = {Dvir, Zeev and Shpilka, Amir},
	Journal = {Combinatorica},
	Number = {3},
	Pages = {305},
	Title = {Towards dimension expanders over finite fields},
	Volume = {31},
	Year = {2011}}

 @article{Balog1994AST,
  title={A statistical theorem of set addition},
  author={Antal Balog and Endre Szemer{\'e}di},
  journal={Combinatorica},
  year={1994},
  volume={14},
  pages={263-268}
}

@article{Gowers1998ANP,
  title={A New Proof of Szemer{\'e}di's Theorem for Arithmetic Progressions of Length Four},
  author={William T. Gowers},
  journal={Geometric \& Functional Analysis GAFA},
  year={1998},
  volume={8},
  pages={529-551}
}

@book{tao_vu_2006, place={Cambridge}, series={Cambridge Studies in Advanced Mathematics}, title={Additive Combinatorics}, DOI={10.1017/CBO9780511755149}, publisher={Cambridge University Press}, author={Tao, Terence and Vu, Van H.}, year={2006}, collection={Cambridge Studies in Advanced Mathematics}}

@article{CG88,
author = {Chor, Benny and Goldreich, Oded},
title = {Unbiased Bits from Sources of Weak Randomness and Probabilistic Communication Complexity},
journal = {SIAM Journal on Computing},
volume = {17},
number = {2},
pages = {230-261},
year = {1988}
}

@InProceedings{GryaznovPT:CCC:2022,
  author =	{Gryaznov, Svyatoslav and Pudl\'{a}k, Pavel and Talebanfard, Navid},
  title =	{{Linear Branching Programs and Directional Affine Extractors}},
  booktitle =	{37th Computational Complexity Conference (CCC 2022)},
  pages =	{4:1--4:16},
  year =	{2022},
  volume =	{234}
}

@INPROCEEDINGS{ChattopadhyayL:focs:2016,
  author={Chattopadhyay, Eshan and Li, Xin},
  booktitle={2016 IEEE 57th Annual Symposium on Foundations of Computer Science (FOCS)}, 
  title={Explicit Non-malleable Extractors, Multi-source Extractors, and Almost Optimal Privacy Amplification Protocols}, 
  year={2016},
  volume={},
  number={},
  pages={158-167},
  doi={10.1109/FOCS.2016.25}}

@techreport{ChattopadhyayL22b,
  author    = {Eshan Chattopadhyay and
               Jyun{-}Jie Liao},
  title     = {Hardness against Linear Branching Programs and More},
  Institution = {Electron. Colloquium Comput. Complex.},
  volume    = {{TR22-153}},
  year      = {2022},
  url       = {https://eccc.weizmann.ac.il/report/2022/153},
}

@inproceedings{DK11,
	Author	= {Evgeny Demenkov and Alexander Kulikov},
	Booktitle = "Proceedings of the 36th international conference on Mathematical foundations of computer science",
	Title	= {An Elementary Proof of 3n-o(n) Lower Bound on the Circuit Complexity of Affine Dispersers},
	pages = {256--265},
	year	= {2011}
}

@INPROCEEDINGS{FGHK15,
  author={Find, Magnus Gausdal and Golovnev, Alexander and Hirsch, Edward A. and Kulikov, Alexander S.},
  booktitle={2016 IEEE 57th Annual Symposium on Foundations of Computer Science (FOCS)}, 
  title={A Better-Than-3n Lower Bound for the Circuit Complexity of an Explicit Function}, 
  year={2016},
  pages={89-98},
  doi={10.1109/FOCS.2016.19}}
  
@inproceedings{LY22,
author = {Li, Jiatu and Yang, Tianqi},
title = {3.1n - o(n) Circuit Lower Bounds for Explicit Functions},
year = {2022},
isbn = {9781450392648},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3519935.3519976},
doi = {10.1145/3519935.3519976},
booktitle = {Proceedings of the 54th Annual ACM SIGACT Symposium on Theory of Computing},
pages = {1180–1193},
numpages = {14},
keywords = {gate elimination, explicit lower bounds, affine dispersers, Boolean circuits},
location = {Rome, Italy},
series = {STOC 2022}
}

@inproceedings{CohenS16,
  author    = {Gil Cohen and
               Igor Shinkar},
  editor    = {Madhu Sudan},
  title     = {The Complexity of {DNF} of Parities},
  booktitle = {Proceedings of the 2016 {ACM} Conference on Innovations in Theoretical
               Computer Science, Cambridge, MA, USA, January 14-16, 2016},
  pages     = {47--58},
  publisher = {{ACM}},
  year      = {2016},
  url       = {https://doi.org/10.1145/2840728.2840734},
  doi       = {10.1145/2840728.2840734},
  timestamp = {Tue, 14 Jun 2022 13:12:41 +0200},
  biburl    = {https://dblp.org/rec/conf/innovations/CohenS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@techreport{Li23,
  author    = {Xin Li},
  title     = {Two Source Extractors for Asymptotically Optimal Entropy, and (Many) More},
  Institution = {Arxiv},
Note = {{\tt https://arxiv.org/abs/2303.06802}},
    Year = {2023},
}


@article{BorodinRS93,
	Author = {Borodin, A. and Razborov, A. and Smolensky, R.},
	Da = {1993/03/01},
	Date-Added = {2023-04-25 22:19:33 +0000},
	Date-Modified = {2023-04-25 22:19:33 +0000},
	Doi = {10.1007/BF01200404},
	Id = {Borodin1993},
	Isbn = {1420-8954},
	Journal = {computational complexity},
	Number = {1},
	Pages = {1--18},
	Title = {On lower bounds for read-k-times branching programs},
	Ty = {JOUR},
	Url = {https://doi.org/10.1007/BF01200404},
	Volume = {3},
	Year = {1993},
	Bdsk-Url-1 = {https://doi.org/10.1007/BF01200404},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/BF01200404}}


@article{ABLAYEV200378,
	Author = {Farid Ablayev and Marek Karpinski},
	Doi = {https://doi.org/10.1016/S0890-5401(03)00118-4},
	Issn = {0890-5401},
	Journal = {Information and Computation},
	Keywords = {Deterministic and randomized branching programs, OBDD, Complexity, Lower bounds, Integer multiplication, Randomized algorithms},
	Number = {1},
	Pages = {78-89},
	Title = {A lower bound for integer multiplication on randomized ordered read-once branching programs},
	Url = {https://www.sciencedirect.com/science/article/pii/S0890540103001184},
	Volume = {186},
	Year = {2003},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0890540103001184},
	Bdsk-Url-2 = {https://doi.org/10.1016/S0890-5401(03)00118-4}}


@inproceedings{DBLP:conf/stoc/BolligW01,
  author       = {Beate Bollig and
                  Philipp Woelfel},
  editor       = {Jeffrey Scott Vitter and
                  Paul G. Spirakis and
                  Mihalis Yannakakis},
  title        = {A read-once branching program lower bound of Omega(2\({}^{\mbox{n/4}}\))
                  for integer multiplication using universal},
  booktitle    = {Proceedings on 33rd Annual {ACM} Symposium on Theory of Computing,
                  July 6-8, 2001, Heraklion, Crete, Greece},
  pages        = {419--424},
  publisher    = {{ACM}},
  year         = {2001},
  url          = {https://doi.org/10.1145/380752.380835},
  doi          = {10.1145/380752.380835},
  timestamp    = {Tue, 06 Nov 2018 11:07:06 +0100},
  biburl       = {https://dblp.org/rec/conf/stoc/BolligW01.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{doi:10.1137/S0097539795290349,
	Author = {Ponzio, Stephen},
	Doi = {10.1137/S0097539795290349},
	Eprint = {https://doi.org/10.1137/S0097539795290349},
	Journal = {SIAM Journal on Computing},
	Number = {3},
	Pages = {798-815},
	Title = {A Lower Bound for Integer Multiplication with Read-Once Branching Programs},
	Url = {https://doi.org/10.1137/S0097539795290349},
	Volume = {28},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1137/S0097539795290349},
	Bdsk-Url-2 = {http://dx.doi.org/10.1137/S0097539795290349}}


@techreport{LiZ23,
  author    = {Xin Li and Yan Zhong},
  title     = {Explicit Directional Affine Extractors and Improved Hardness for Linear Branching Programs},
  Institution = {Arxiv},
Note = {{\tt https://arxiv.org/abs/2304.11495}},
    Year = {2023},
}


@inproceedings{Hastad86,
  author    = {Johan H{\aa}stad},
  editor    = {Juris Hartmanis},
  title     = {Almost Optimal Lower Bounds for Small Depth Circuits},
  booktitle = {Proceedings of the 18th Annual {ACM} Symposium on Theory of Computing,
               May 28-30, 1986, Berkeley, California, {USA}},
  pages     = {6--20},
  publisher = {{ACM}},
  year      = {1986},
  url       = {https://doi.org/10.1145/12130.12132},
  doi       = {10.1145/12130.12132},
  timestamp = {Sun, 02 Jun 2019 21:10:31 +0200},
  biburl    = {https://dblp.org/rec/conf/stoc/Hastad86.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{ChattopadhyayL22,
  author    = {Eshan Chattopadhyay and
               Jyun{-}Jie Liao},
  editor    = {Stefano Leonardi and
               Anupam Gupta},
  title     = {Extractors for sum of two sources},
  booktitle = {{STOC} '22: 54th Annual {ACM} {SIGACT} Symposium on Theory of Computing,
               Rome, Italy, June 20 - 24, 2022},
  pages     = {1584--1597},
  publisher = {{ACM}},
  year      = {2022},
  url       = {https://doi.org/10.1145/3519935.3519963},
  doi       = {10.1145/3519935.3519963},
  timestamp = {Tue, 27 Dec 2022 09:06:31 +0100},
  biburl    = {https://dblp.org/rec/conf/stoc/ChattopadhyayL22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ChattopadhyayL16,
  author    = {Eshan Chattopadhyay and
               Xin Li},
  editor    = {Daniel Wichs and
               Yishay Mansour},
  title     = {Extractors for sumset sources},
  booktitle = {Proceedings of the 48th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC}, Cambridge, MA, USA, June 18-21, 2016},
  pages     = {299--311},
  publisher = {{ACM}},
  year      = {2016},
  url       = {https://doi.org/10.1145/2897518.2897643},
  doi       = {10.1145/2897518.2897643},
  timestamp = {Tue, 06 Nov 2018 11:07:05 +0100},
  biburl    = {https://dblp.org/rec/conf/stoc/ChattopadhyayL16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@INPROCEEDINGS{ChattopadhyayGL:focs:2021,
  author={Chattopadhyay, Eshan and Goodman, Jesse and Liao, Jyun-Jie},
  booktitle={2021 IEEE 62nd Annual Symposium on Foundations of Computer Science (FOCS)}, 
  title={Affine Extractors for Almost Logarithmic Entropy}, 
  year={2022},
  volume={},
  number={},
  pages={622-633},
  doi={10.1109/FOCS52979.2021.00067}}


@InProceedings{CohenT:random:2015,
    author = {Cohen, Gil and Tal, Avishay},
    title = {Two Structural Results for Low Degree Polynomials and Applications},
    booktitle =	{Approximation, Randomization, and Combinatorial Optimization. Algorithms and Techniques, APPROX/RANDOM 2015},
    year={2015}
}

@article{DodisORS08,
author = {Dodis, Yevgeniy and Ostrovsky, Rafail and Reyzin, Leonid and Smith, Adam},
title = {Fuzzy Extractors: How to Generate Strong Keys from Biometrics and Other Noisy Data},
journal = {SIAM Journal on Computing},
volume = {38},
number = {1},
pages = {97-139},
year = {2008}
}

@article{Wegener88,
  author    = {Ingo Wegener},
  title     = {On the complexity of branching programs and decision trees for clique
               functions},
  journal   = {J. {ACM}},
  volume    = {35},
  number    = {2},
  pages     = {461--471},
  year      = {1988},
  url       = {https://doi.org/10.1145/42282.46161},
  doi       = {10.1145/42282.46161},
  timestamp = {Wed, 14 Nov 2018 10:35:26 +0100},
  biburl    = {https://dblp.org/rec/journals/jacm/Wegener88.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Zak84,
  author    = {Stanislav Z{\'{a}}k},
  editor    = {Michal Chytil and
               V{\'{a}}clav Koubek},
  title     = {An Exponential Lower Bound for One-Time-Only Branching Programs},
  booktitle = {Mathematical Foundations of Computer Science 1984, Praha, Czechoslovakia,
               September 3-7, 1984, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {176},
  pages     = {562--566},
  publisher = {Springer},
  year      = {1984},
  url       = {https://doi.org/10.1007/BFb0030340},
  doi       = {10.1007/BFb0030340},
  timestamp = {Tue, 14 May 2019 10:00:37 +0200},
  biburl    = {https://dblp.org/rec/conf/mfcs/Zak84.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/fct/Dunne85,
  author    = {Paul E. Dunne},
  editor    = {Lothar Budach},
  title     = {Lower bounds on the complexity of 1-time only branching programs},
  booktitle = {Fundamentals of Computation Theory, {FCT} '85, Cottbus, GDR, September
               9-13, 1985},
  series    = {Lecture Notes in Computer Science},
  volume    = {199},
  pages     = {90--99},
  publisher = {Springer},
  year      = {1985},
  url       = {https://doi.org/10.1007/BFb0028795},
  doi       = {10.1007/BFb0028795},
  timestamp = {Tue, 14 May 2019 10:00:53 +0200},
  biburl    = {https://dblp.org/rec/conf/fct/Dunne85.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tcs/Jukna88,
  author    = {Stasys Jukna},
  title     = {Entropy of Contact Circuits and Lower Bounds on Their Complexity},
  journal   = {Theor. Comput. Sci.},
  volume    = {57},
  pages     = {113--129},
  year      = {1988},
  url       = {https://doi.org/10.1016/0304-3975(88)90166-1},
  doi       = {10.1016/0304-3975(88)90166-1},
  timestamp = {Sun, 02 Oct 2022 15:50:31 +0200},
  biburl    = {https://dblp.org/rec/journals/tcs/Jukna88.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tcs/KrauseMW91,
  author    = {Matthias Krause and
               Christoph Meinel and
               Stephan Waack},
  title     = {Separating the Eraser Turing Machine Classes L{\_}e, NL{\_}e, co-NL{\_}e
               and P{\_}e},
  journal   = {Theor. Comput. Sci.},
  volume    = {86},
  number    = {2},
  pages     = {267--275},
  year      = {1991},
  url       = {https://doi.org/10.1016/0304-3975(91)90021-S},
  doi       = {10.1016/0304-3975(91)90021-S},
  timestamp = {Wed, 17 Feb 2021 21:59:27 +0100},
  biburl    = {https://dblp.org/rec/journals/tcs/KrauseMW91.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Simon1992ANL,
  title={A New Lower Bound Theorem for Read-Only-Once Branching Programs and its Applications},
  author={Janos Simon and Mario Szegedy},
  booktitle={Advances In Computational Complexity Theory},
  year={1992}
}

@article{savitch1970relationships,
  title={Relationships between nondeterministic and deterministic tape complexities},
  author={Savitch, Walter J},
  journal={Journal of computer and system sciences},
  volume={4},
  number={2},
  pages={177--192},
  year={1970},
  publisher={Elsevier}
}

 @article{DBLP:journals/ipl/Gal97,
  author    = {Anna G{\'{a}}l},
  title     = {A Simple Function that Requires Exponential Size Read-Once Branching
               Programs},
  journal   = {Inf. Process. Lett.},
  volume    = {62},
  number    = {1},
  pages     = {13--16},
  year      = {1997},
  url       = {https://doi.org/10.1016/S0020-0190(97)00041-0},
  doi       = {10.1016/S0020-0190(97)00041-0},
  timestamp = {Fri, 26 May 2017 22:54:41 +0200},
  biburl    = {https://dblp.org/rec/journals/ipl/Gal97.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ipl/BolligW98,
  author    = {Beate Bollig and
               Ingo Wegener},
  title     = {A Very Simple Function that Requires Exponential Size Read-Once Branching
               Programs},
  journal   = {Inf. Process. Lett.},
  volume    = {66},
  number    = {2},
  pages     = {53--57},
  year      = {1998},
  url       = {https://doi.org/10.1016/S0020-0190(98)00042-8},
  doi       = {10.1016/S0020-0190(98)00042-8},
  timestamp = {Fri, 26 May 2017 22:54:41 +0200},
  biburl    = {https://dblp.org/rec/journals/ipl/BolligW98.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{AndreevBCR99,
  author    = {Alexander E. Andreev and
               Juri L. Baskakov and
               Andrea E. F. Clementi and
               Jos{\'{e}} D. P. Rolim},
  editor    = {Jir{\'{\i}} Wiedermann and
               Peter van Emde Boas and
               Mogens Nielsen},
  title     = {Small Pseudo-Random Sets Yield Hard Functions: New Tight Explict Lower
               Bounds for Branching Programs},
  booktitle = {Automata, Languages and Programming, 26th International Colloquium,
               ICALP'99, Prague, Czech Republic, July 11-15, 1999, Proceedings},
  series    = {Lecture Notes in Computer Science},
  volume    = {1644},
  pages     = {179--189},
  publisher = {Springer},
  year      = {1999},
  url       = {https://doi.org/10.1007/3-540-48523-6\_15},
  doi       = {10.1007/3-540-48523-6\_15},
  timestamp = {Tue, 14 May 2019 10:00:44 +0200},
  biburl    = {https://dblp.org/rec/conf/icalp/AndreevBCR99.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Yehudayoff11,
    Author = { Amir Yehudayoff},
    Journal = {Combinatorica},
    Volume = 31,
    number = {2},
    pages = {245--256},
    Title = {Affine extractors over prime fields},
     Year = 2011}
     
@article{DBLP:journals/tcs/Kabanets03,
  author    = {Valentine Kabanets},
  title     = {Almost k-wise independence and hard Boolean functions},
  journal   = {Theor. Comput. Sci.},
  volume    = {297},
  number    = {1-3},
  pages     = {281--295},
  year      = {2003},
  url       = {https://doi.org/10.1016/S0304-3975(02)00643-6},
  doi       = {10.1016/S0304-3975(02)00643-6},
  timestamp = {Wed, 17 Feb 2021 21:57:41 +0100},
  biburl    = {https://dblp.org/rec/journals/tcs/Kabanets03.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Nechiporuk66,
author = {E. I. Nechiporuk},
title = {On a boolean function},
journal = {Doklady of the Academy of Sciences of the USSR},
volume = {164},
number = {4},
pages = {765--766},
year = {1966}
}

@inproceedings{Li:stoc:17,
author = {Li, Xin},
title = {Improved Non-Malleable Extractors, Non-Malleable Codes and Independent Source Extractors},
year = {2017},
isbn = {9781450345286},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
 booktitle = {Proceedings of the 49th Annual {ACM} {SIGACT} Symposium on Theory
               of Computing, {STOC} 2017, Montreal, QC, Canada, June 19-23, 2017},
pages = {1144–1156},
numpages = {13},
keywords = {extractor, privacy, coding, non-malleable},
location = {Montreal, Canada},
series = {STOC 2017}
}

@phdthesis{Vazirani86,
author = {Vazirani, Umesh Virkumar},
title = {Randomness, Adversaries and Computation (Random Polynomial Time)},
year = {1986},
publisher = {University of California, Berkeley},
school = {University of California, Berkeley},
note = {AAI8718194}
}

@inproceedings{Rao:ccc:09,
author = {Rao, Anup},
title = {Extractors for Low-Weight Affine Sources},
year = {2009},
isbn = {9780769537177},
publisher = {IEEE Computer Society},
booktitle = {Proceedings of the 2009 24th Annual IEEE Conference on Computational Complexity},
pages = {95–101},
numpages = {7},
keywords = {Extractors, Exposure Resilient Cryptography, Bit-Fixing Sources, Affine Sources},
series = {CCC '09}
}

@inproceedings{CGL:stoc:16,
author = {Chattopadhyay, Eshan and Goyal, Vipul and Li, Xin},
title = {Non-Malleable Extractors and Codes, with Their Many Tampered Extensions},
year = {2016},
isbn = {9781450341325},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the Forty-Eighth Annual ACM Symposium on Theory of Computing},
pages = {285–298},
numpages = {14},
keywords = {Non-Malleable Extractors, Non-Malleable Codes, Randomness Extractor, Pseudorandomness, Privacy Amplification},
location = {Cambridge, MA, USA},
series = {STOC '16}
}

@inproceedings{beame1989general,
  title={A general sequential time-space tradeoff for finding unique elements},
  author={Beame, Paul},
  booktitle={Proceedings of the twenty-first annual ACM symposium on Theory of computing},
  pages={197--203},
  year={1989}
}

@inproceedings{pippenger1979simultaneous,
  title={On simultaneous resource bounds},
  author={Pippenger, Nicholas},
  booktitle={20th Annual Symposium on Foundations of Computer Science (sfcs 1979)},
  pages={307--311},
  year={1979},
  organization={IEEE}
}

@inproceedings{saha17,
	title={Fast \& Space-Efficient Approximations of Language Edit Distance and {RNA} Folding: An Amnesic Dynamic Programming Approach},
	author={Saha, Barna},
	booktitle={FOCS},
	year={2017}
}

@inproceedings{sun2007communication,
	title={The communication and streaming complexity of computing the longest common and increasing subsequences},
	author={Sun, Xiaoming and Woodruff, David P},
	booktitle={Proceedings of the eighteenth annual ACM-SIAM symposium on Discrete algorithms},
	pages={336--345},
	year={2007}
}

@article{Ailon2007EstimatingTD,
  title={Estimating the distance to a monotone function},
  author={Nir Ailon and Bernard Chazelle and Seshadhri Comandur and Ding Liu},
  journal={Random Structures \& Algorithms},
  year={2007},
  volume={31}
}

@InProceedings{li_et_al:LIPIcs.FSTTCS.2021.27,
  author =	{Li, Xin and Zheng, Yu},
  title =	{{Lower Bounds and Improved Algorithms for Asymmetric Streaming Edit Distance and Longest Common Subsequence}},
  booktitle =	{FSTTCS 2021}
}

@article{gal2010lower,
	title={Lower bounds on streaming algorithms for approximating the length of the longest increasing subsequence},
	author={G{\'a}l, Anna and Gopalan, Parikshit},
	journal={SIAM Journal on Computing},
	volume={39},
	number={8},
	pages={3463--3479},
	year={2010},
	publisher={SIAM}
}

@inproceedings{ergun2008distance,
  title={On distance to monotonicity and longest increasing subsequence of a data stream},
  author={Ergun, Funda and Jowhari, Hossein},
  booktitle={Proceedings of the nineteenth annual ACM-SIAM symposium on Discrete algorithms},
  pages={730--736},
  year={2008}
}


@inproceedings{DBLP:conf/soda/GopalanJKK07,
	author    = {Parikshit Gopalan and
	T. S. Jayram and
	Robert Krauthgamer and
	Ravi Kumar},
	title     = {Estimating the sortedness of a data stream},
	booktitle = {SODA},
	year={2007}
}

@article{haastad2007randomized,
  title={The randomized communication complexity of set disjointness},
  author={H{\aa}stad, Johan and Wigderson, Avi},
  journal={Theory of Computing},
  volume={3},
  number={1},
  pages={211--219},
  year={2007},
  publisher={Theory of Computing Exchange}
}


@article{doi:10.1137/1004036,
	Author = {Mallows, C. L.},
	Doi = {10.1137/1004036},
	Eprint = {https://doi.org/10.1137/1004036},
	Journal = {SIAM Review},
	Number = {2},
	Pages = {148-149},
	Title = {Patience Sorting},
	Url = {https://doi.org/10.1137/1004036},
	Volume = {4},
	Year = {1962},
	Bdsk-Url-1 = {https://doi.org/10.1137/1004036},
	Bdsk-Url-2 = {http://dx.doi.org/10.1137/1004036}}


@article{Hammersley72,
  title={A few seedlings of research},
  author={John Hammersley},
  journal={Proc. Sixth Berkeley Symp. Math. Statist.
and Probability},

  pages={345--394},
  year={1972}
}

@inproceedings{cheng_et_al:LIPIcs.ICALP.2021.54,
  title={Streaming and Small Space Approximation Algorithms for Edit Distance and Longest Common Subsequence},
  author={Cheng, Kuan and Farhadi, Alireza and Hajiaghayi, MohammadTaghi and Jin, Zhengzhong and Li, Xin and Rubinstein, Aviad and Seddighin, Saeed and Zheng, Yu},
  booktitle={ICALP 2021},
  year={2021}
}
% year={2021}
% organization={Schloss Dagstuhl-Leibniz-Zentrum f{\"u}r Informatik}

@INPROCEEDINGS{9996890,
  author={Andoni, Alexandr and Nosatzki, Negev Shekel and Sinha, Sandip and Stein, Clifford},
  booktitle={2022 IEEE 63rd Annual Symposium on Foundations of Computer Science (FOCS)}, 
  title={Estimating the Longest Increasing Subsequence in Nearly Optimal Time}, 
  year={2022},
  volume={},
  number={},
  pages={708-719},
  doi={10.1109/FOCS54457.2022.00073}}

@inproceedings{DBLP:conf/soda/MitzenmacherS21,
  author       = {Michael Mitzenmacher and
                  Saeed Seddighin},
  editor       = {D{\'{a}}niel Marx},
  title        = {Improved Sublinear Time Algorithm for Longest Increasing Subsequence},
  booktitle    = {Proceedings of the 2021 {ACM-SIAM} Symposium on Discrete Algorithms,
                  {SODA} 2021, Virtual Conference, January 10 - 13, 2021},
  pages        = {1934--1947},
  publisher    = {{SIAM}},
  year         = {2021},
  url          = {https://doi.org/10.1137/1.9781611976465.115},
  doi          = {10.1137/1.9781611976465.115},
  timestamp    = {Thu, 15 Jul 2021 13:49:01 +0200},
  biburl       = {https://dblp.org/rec/conf/soda/MitzenmacherS21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/focs/RubinsteinSSS19,
  author       = {Aviad Rubinstein and
                  Saeed Seddighin and
                  Zhao Song and
                  Xiaorui Sun},
  editor       = {David Zuckerman},
  title        = {Approximation Algorithms for {LCS} and {LIS} with Truly Improved Running
                  Times},
  booktitle    = {{FOCS}
                  2019, Baltimore, Maryland, USA, November 9-12, 2019},
  pages        = {1121--1145},
  publisher    = {{IEEE} Computer Society},
  year         = {2019},
  url          = {https://doi.org/10.1109/FOCS.2019.00071},
  doi          = {10.1109/FOCS.2019.00071},
  timestamp    = {Sat, 05 Dec 2020 12:59:44 +0100},
  biburl       = {https://dblp.org/rec/conf/focs/RubinsteinSSS19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{saks2013space,
  title={Space efficient streaming algorithms for the distance to monotonicity and asymmetric edit distance},
  author={Saks, Michael and Seshadhri, C},
  booktitle={SODA},
  year={2013}
}


@inproceedings{im2017efficient,
  title={Efficient massively parallel methods for dynamic programming},
  author={Im, Sungjin and Moseley, Benjamin and Sun, Xiaorui},
  booktitle={Proceedings of the 49th Annual ACM SIGACT Symposium on Theory of Computing},
  pages={798--811},
  year={2017},
  organization={ACM}
}

@inproceedings{DBLP:conf/stoc/KociumakaS21,
  author       = {Tomasz Kociumaka and
                  Saeed Seddighin},
  editor       = {Samir Khuller and
                  Virginia Vassilevska Williams},
  title        = {Improved dynamic algorithms for longest increasing subsequence},
  booktitle    = {{STOC} '21: 53rd Annual {ACM} {SIGACT} Symposium on Theory of Computing,
                  Virtual Event, Italy, June 21-25, 2021},
  pages        = {640--653},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3406325.3451026},
  doi          = {10.1145/3406325.3451026},
  timestamp    = {Sat, 08 Jan 2022 02:24:28 +0100},
  biburl       = {https://dblp.org/rec/conf/stoc/KociumakaS21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/stoc/MitzenmacherS20,
  author       = {Michael Mitzenmacher and
                  Saeed Seddighin},
  editor       = {Konstantin Makarychev and
                  Yury Makarychev and
                  Madhur Tulsiani and
                  Gautam Kamath and
                  Julia Chuzhoy},
  title        = {Dynamic algorithms for {LIS} and distance to monotonicity},
  booktitle    = {Proccedings of the 52nd Annual {ACM} {SIGACT} Symposium on Theory
                  of Computing, {STOC} 2020, Chicago, IL, USA, June 22-26, 2020},
  pages        = {671--684},
  publisher    = {{ACM}},
  year         = {2020},
  url          = {https://doi.org/10.1145/3357713.3384240},
  doi          = {10.1145/3357713.3384240},
  timestamp    = {Sat, 08 Jan 2022 02:24:27 +0100},
  biburl       = {https://dblp.org/rec/conf/stoc/MitzenmacherS20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/stoc/GawrychowskiJ21,
  author       = {Pawel Gawrychowski and
                  Wojciech Janczewski},
  editor       = {Samir Khuller and
                  Virginia Vassilevska Williams},
  title        = {Fully dynamic approximation of {LIS} in polylogarithmic time},
  booktitle    = {{STOC} '21: 53rd Annual {ACM} {SIGACT} Symposium on Theory of Computing,
                  Virtual Event, Italy, June 21-25, 2021},
  pages        = {654--667},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3406325.3451137},
  doi          = {10.1145/3406325.3451137},
  timestamp    = {Thu, 14 Oct 2021 09:45:35 +0200},
  biburl       = {https://dblp.org/rec/conf/stoc/GawrychowskiJ21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inbook{doi:10.1137/1.9781611973730.83,
	Author = {Timothy Naumovitz and Michael Saks},
	Booktitle = {Proceedings of the 2015 Annual ACM-SIAM Symposium on Discrete Algorithms (SODA)},
	Doi = {10.1137/1.9781611973730.83},
	Eprint = {https://epubs.siam.org/doi/pdf/10.1137/1.9781611973730.83},
	Pages = {1252-1262},
	Title = {A polylogarithmic space deterministic streaming algorithm for approximating distance to monotonicity},
	Url = {https://epubs.siam.org/doi/abs/10.1137/1.9781611973730.83},
	Bdsk-Url-1 = {https://epubs.siam.org/doi/abs/10.1137/1.9781611973730.83},
	Bdsk-Url-2 = {http://dx.doi.org/10.1137/1.9781611973730.83},
 year={2015}}

@article{doi:10.1137/130942152,
	Author = {Saks, M. and Seshadhri, C.},
	Doi = {10.1137/130942152},
	Eprint = {https://doi.org/10.1137/130942152},
	Journal = {SIAM Journal on Computing},
	Number = {2},
	Pages = {774-823},
	Title = {Estimating the Longest Increasing Sequence in Polylogarithmic Time},
	Url = {https://doi.org/10.1137/130942152},
	Volume = {46},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1137/130942152},
	Bdsk-Url-2 = {http://dx.doi.org/10.1137/130942152}}


@article{Mallows73,
  title={Patience sorting},
  author={C. L. Mallows.},
  journal={Bulletin of the Institute of Mathematics and its Applications},
  volume       = {9},
  pages={216--224},
  year={1973}
}

@article{DBLP:journals/mst/KiyomiOOST20,
  author       = {Masashi Kiyomi and
                  Hirotaka Ono and
                  Yota Otachi and
                  Pascal Schweitzer and
                  Jun Tarui},
  title        = {Space-Efficient Algorithms for Longest Increasing Subsequence},
  journal      = {Theory Comput. Syst.},
  volume       = {64},
  number       = {3},
  pages        = {522--541},
  year         = {2020},
  url          = {https://doi.org/10.1007/s00224-018-09908-6},
  doi          = {10.1007/s00224-018-09908-6},
  timestamp    = {Thu, 23 Jun 2022 20:05:15 +0200},
  biburl       = {https://dblp.org/rec/journals/mst/KiyomiOOST20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{roughgarden2016communication,
  author       = {Tim Roughgarden},
  title        = {Communication Complexity (for Algorithm Designers)},
  journal      = {CoRR},
  volume       = {abs/1509.06257},
  year         = {2015},
  url          = {http://arxiv.org/abs/1509.06257},
  eprinttype    = {arXiv},
  eprint       = {1509.06257},
  timestamp    = {Mon, 13 Aug 2018 16:46:03 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/Roughgarden15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

==> streaming_comparison.tex <==
\section{Lower Bounds for Comparison Based Streaming LIS}


